A crossover between open quantum random walks to quantum walks

We propose an intermediate walk continuously connecting an open quantum random walk and a quantum walk with parameters $M\in \mathbb{N}$ controlling a decoherence effect; if $M=1$, the walk coincides with an open quantum random walk, while $M=\infty$, the walk coincides with a quantum walk. We define a measure which recovers usual probability measures on $\mathbb{Z}$ for $M=\infty$ and $M=1$ and we observe intermediate behavior through numerical simulations for varied positive values $M$. In the case for $M=2$, we analytically show that a typical behavior of quantum walks appears even in a small gap of the parameter from the open quantum random walk. More precisely, we observe both the ballistically moving towards left and right sides and localization of this walker simultaneously. The analysis is based on Kato's perturbation theory for linear operator. We futher analyze this limit theorem in more detail and show that the above three modes are described by Gaussian distributions.

==> figs/numerics.tex <==

In this section we summarize numerical observations for various $M$ including $M=1,2$ visualizing the connection of the nature among random walks and quantum walks through our proposed model.
Here we demonstrate the following objects:
\begin{itemize}
\item Distributions of walkers for each $M$, restricted to the diagonal $x=y$.
\item $\log$-plot of the position of peaks off the diagonal (for each $M$).
\item The height of peaks on the edge and the center as well as their ratio.
\item Effective time of interference of the wall.
\end{itemize}

In the whole computations in this section, we fix the initial state $\phi$ as
\begin{equation*}
\phi = \phi_{1}\otimes \phi_1,\quad \text{ where } \quad \phi_1 = \begin{pmatrix}
1/2\\
1/2
\end{pmatrix}.
\end{equation*}
Note that all figures in this section is normalized so that the all walkers are inside $\bar x\in [-1,1]$.
More precisely, we draw all distributions of walkers as relationships between $\bar x \equiv x/N$ and $N\rho_{n+1}^{QW}(\bar x)$ for a given time $N$.

\subsection{Distributions of walkers for each $M$, restricted to the diagonal $x=y$}
First we show asymptotic distribution of walkers for each $M$.
We first study typical behavior of the present model.
Figure \ref{fig-dynamics_sample} shows the distribution with relatively large $M$. 
In the present situation, namely the walker does not arrive at the boundary, the distribution is like the Hadamard's walk.

\begin{remark}
In Figures \ref{fig-dynamics_sample}-\ref{fig-dynamics_long_varM_2}, the scalings $(x,y) \mapsto (x/n, y/n)$ and $\phi_n \mapsto n\phi_n$ are applied for visibility.
The former is operated so that the support of walker density distribution is included in $[-1,1]$. 
The latter is then operated so that the integral of walker density over $[-1,1]$ is kept under the present transformation.
\end{remark}

\begin{figure}[htbp]
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=6.0cm]{figs/3d_M=201_T=100.png}
(a)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=6.0cm]{figs/diag_M=201_T=100.png}
(b)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=6.0cm]{figs/diag_M=500_T=200.png}
(c)
\end{minipage}
\caption{Typical dynamics of the present model with large $M$}
\label{fig-dynamics_sample}
(a): $3$-dimensional plot of distribution under $n=100$ iterations and $M=201$. 
Black solid lines denote the boundary of the domain.
(b): Plot of $\rho_{100}(x)$ with $M=201$. 
(c): Plot of $\rho_{200}(x)$ with $M=500$. 
From (b) and (c), we see that the distribution of $\rho_n$ behaves like the well-known Hadamard walk.
\end{figure}


Next we change the width $M$ and the iteration step $N$ so that $N$ is sufficiently larger than $M$, and compute the dynamics.
Figures \ref{fig-dynamics_sample_varM_1}-\ref{fig-dynamics_sample_varM_2} show the distribution of walkers $\|\phi(x)\|^2$ at each $x$ after $n=100$ iterations, restricted to the diagonal line $x=y$.
As indicated in Section \ref{}, walkers distribute like random walks when $M=1$, which is seen in Figure \ref{fig-dynamics_sample_varM_1}-(a).
When we change $M$ into $2$, the quantum-walk-like interaction comes into play, as seen in Figure \ref{fig-dynamics_sample_varM_1}-(b).
More precisely, the edge-like distributions arise in both sides of the central distribution.
%The limiting width of the side peak is different from that of the center, whereas it is not zero.
As $M$ increases, non-trivial distributions arise between the center and the size peak.
When $M=3$ (Figure \ref{fig-dynamics_sample_varM_1}-(c)), the height of peaks among the center and sides becomes drastically different, unlike the case $M=2$.
Moreover, we also observe the negative-value distribution when $M\geq 3$.
This tendency persists for relatively large $M$, while it converges to zero as $M$ becomes larger.
Finally, the distribution of walkers converges to that for the Hadamard walk as $M$ becomes larger and larger.
We have also studied long-time behavior of these distributions.
Figures \ref{fig-dynamics_long_varM_1}-\ref{fig-dynamics_long_varM_2} show the distribution of walkers after $n=10000$ iterations with $M=1,2,3,5,10, 51$.
We see that the tendency of walker distributions is similar to the corresponding shorter time evolution results (Figures \ref{fig-dynamics_sample_varM_1}-\ref{fig-dynamics_sample_varM_2}), while we can see the behavior clearer.
For example, the side peaks arise when $M\geq 2$, but the heights of peaks look almost identical in the case $M=2$, while they are significantly different when $M\geq 3$.
As $M$ increases, the number of localized islands increases and accumulated to construct Hadamard walk-like limiting behavior.



\begin{figure}[htbp]
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=1_T=100.png}
(a)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=2_T=100.png}
(b)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=3_T=100.png}
(c)
\end{minipage}
\caption{Graph of $\rho_{100}(x)$ for various $M$: part 1}
\label{fig-dynamics_sample_varM_1}
(a): $M=1$.
(b): $M=2$.
(c): $M=3$.
\end{figure}

\begin{figure}[htbp]
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=5_T=100.png}
(a)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=10_T=100.png}
(b)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=51_T=100.png}
(c)
\end{minipage}
\caption{Graph of $\rho_{100}(x)$ for various $M$: part 2}
\label{fig-dynamics_sample_varM_2}
(a): $M=5$.
(b): $M=10$.
(c): $M=51$.
\end{figure}


\begin{figure}[htbp]
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=1_T=10000.png}
(a)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=2_T=10000.png}
(b)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=3_T=10000.png}
(c)
\end{minipage}
\caption{Graph of $\rho_{10000}(x)$ for various $M$: part 1}
\label{fig-dynamics_long_varM_1}
(a): $M=1$.
(b): $M=2$.
(c): $M=3$.
\end{figure}

\begin{figure}[htbp]
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=5_T=10000.png}
(a)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=10_T=10000.png}
(b)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/diag_M=51_T=10000.png}
(c)
\end{minipage}
\caption{Graph of $\rho_{10000}(x)$ for various $M$: part 2}
\label{fig-dynamics_long_varM_2}
(a): $M=5$.
(b): $M=10$.
(c): $M=51$.
\end{figure}



\subsection{Influence of boundary on dynamics}
Next we study the influence of boundary on walkers.
First we fix $n=100$.
Recall that there is no influence of the boundary on walkers when $M$ is sufficiently large, say $M=201$ for $n=100$ and $M=500$ for $n=200$.
Figure \ref{fig-wall} shows the walker distributions with various $M$ in $3$-dimensional visualizations so that influence of the wall is easily visible.
If $M$ is relatively large, we can see no changes among them, which indicates that the influence of the wall on the dynamics does not arrive at the distribution on the diagonal.
On the other hand, if $M$ is smaller than $70$, the interference becomes visible at the center when $n=100$.
As $M$ decreases, the density matrix in the interior is localized and several peaks are observed to make a fringe pattern.
As $M$ decreases further, such localized peaks decay and decrease, and finally, the distribution becomes the Gaussian distribution as $M\to 1$.


\begin{figure}[htbp]
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=7.5cm]{figs/3d_M=101_T=100.png}
(a)
\end{minipage}
\begin{minipage}{0.5\hsize}
\centering
\includegraphics[width=7.5cm]{figs/3d_M=21_T=100.png}
(b)
\end{minipage}\\
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/3d_M=10_T=100.png}
(c)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/3d_M=2_T=100.png}
(d)
\end{minipage}
\begin{minipage}{0.33\hsize}
\centering
\includegraphics[width=5.5cm]{figs/3d_M=1_T=100.png}
(e)
\end{minipage}
\caption{Influence of boundary}
\label{fig-wall}
Black solid lines denote the wall.
(a): $M=101$. Walkers are affected by the wall, while the effect is invisible clearly on the diagonal.
(b): $M=21$. 
Interference of the wall becomes clearly visible, which creates a fringe pattern.
(c): $M=10$. 
Visible fringe patterns become coarser, compared with the case $M=21$.
(d): $M=2$. 
We can observe only three islands. (cf. Figure \ref{fig-dynamics_sample_varM_1}-(b))
(e): $M=1$. 
Walkers accumulate at the center.
In other words, no walkers spread far from the center.
(cf. Figure \ref{fig-dynamics_sample_varM_1}-(a))
\end{figure}


\par
To see the influence of the boundary more precisely, we pay attention to the presence of negative distributions. 
In Figure \ref{fig-dynamics_sample}, we cannot see positions where $\rho_n(x)$ becomes negative, in which case $M$ is relatively large so that the walker does not arrive at the boundary.
On the other hand, in the case that $M$ is relatively small compared with time step $N$, we see negative value distributions of $\rho_n(x)$ separating \lq\lq islands" of distributions attaining positive values (See Figures \ref{fig-dynamics_sample_varM_1}-\ref{fig-dynamics_long_varM_2}), which make fringe patterns in Figure \ref{fig-wall}.
We then see the presence of negative values in $\{\rho_n(x)\}$ as the onset of the influence of the boundary.
To see the tendency precisely, we define the critical time $n_{crit} = n_{crit}(M)$ as follows:
\begin{equation}
\label{n_crit}
n_{crit}(M) := \sup\{n \mid \rho_{\tilde n}(x) \geq 0 \text{ for all $x\in \mathbb{Z}$ and ${\tilde n}\in \{0,1,\cdots, n\}$} \}.
\end{equation}
Figure \ref{fig-critical-N} shows the graphs of $n_{crit}(M)$, which indicates that $n_{crit}(M)$ is almost proportional to $M$ whose slope depends on whether $M$ is even or odd. 
More precisely, we have
\begin{equation*}
n_{crit}(M) \approx
\begin{cases}
3M & \text{$M$ is even},\\
2M & \text{$M$ is odd}.
\end{cases}
\end{equation*}

\begin{figure}[htbp]
\centering
\includegraphics[width=7.5cm]{figs/critical.png}
\caption{Graph of $n_{crit}(M)$ in (\ref{n_crit})}
\label{fig-critical-N}
Horizontal: $M$. Vertical: $n_{crit}(M)$.
Red: plot of $n_{crit}$ for even $M$. 
Namely $n_{crit}(M)$ as a function of only even $M$. 
Blue: plot of $n_{crit}$ for odd $M$ in the similar manner to the red curve. 
\end{figure}






\subsection{Characteristics of off-diagonal peaks}
%Position and height of off-diagonal peaks}
As $M$ increases, the limiting behavior of walker's distribution looks like the Hadamard-type quantum walk.
Here we study several characteristics of distributions to see how close the limiting behavior is to the Hadamard walk.
There are several well-known characteristics of asymptotic behavior in quantum walks such as Hadamard's one (e.g. \cite{Sunada_Tate2012}).
We then study the following values as a function of $n$:
\begin{itemize}
\item the position $\bar x^{\max}_{n, M}$ where the density attains the maximal value,
\item ratio of the height of $\rho_n(0)$ to $\rho_n(\bar x^{\max}_{n, M})$,
\item asymptotic size of tail outside the limiting support $d_n$,
\item decay rate of $\rho_n(0)$ as $n\to \infty$,
\item decay rate of $\rho_n(\bar x^{\max}_{n, M})$ as $n\to \infty$,
\end{itemize}
whose precise definitions are shown below.
Note that all these values can depend on $M$.
These values can {\em quantitatively} characterize the closeness of the limiting behavior of the present model to well-known quantum walks.
In all computation results we show below, we have fixed $n = 5000$ and note that the corresponding values are almost the same between $5000 \leq 10000$.

%%%%
\subsubsection{The position of the density attaining the maximal value}
Looking at all figures in the previous subsections, we see that the leftmost and rightmost peaks of distributions of walkers rarely change as $M$ increases.
The present step is to study the peak position more precisely.
To this end, we extract the position of peaks and its time evolution.
We have computed the peak position of walker distributions outside the center distribution by determining
\begin{equation}
\label{position}
\bar x^{\max}_{n, M} :=\left\{ \bar x \in [\delta,1] \mid \rho_{n}^{QW}(\bar x) = \max_{\bar x\in [\delta,1]} \rho_{n}^{QW}(x)\right\}.
\end{equation}
As a sample result, we have calculated $\left\{\bar x^{\max}_{5000, M} \right\}$ for various $M$. 
Here $\delta > 0$ is a parameter sufficiently small so that the random-walk-like distribution is concentrated on the interval $(-\delta, \delta)$.
Note that each sequence $\left\{\bar x^{\max}_{n, M}\right\}_{n\geq 1}$ is also parameterized by the width $M$ of the stripe.
The sequence $\left\{\bar x^{\max}_{n, 2}\right\}_{n\geq 1}$ converges to $1/\sqrt{3}$, while $\left\{\bar x^{\max}_{n, 3}\right\}_{n\geq 1}$ to $0.64$.
Approximate values of $\bar x^{\max}_{n, M}$ during our computations are summarized in Table \ref{Table-ch1}.
As $M$ increases, the sequence $\left\{\bar x^{\max}_{N, M}\right\}_{M\geq 1}$ becomes distributed around $0.69\sim 0.71$.
This observation shows that the walker spreads depending linearly on $n$ like quantum walks, while the rate of linearity have an influence on the wall. 
More precisely, the thinner the stripe is, the smaller the rate is.
It is also noted that our numerical result for $M=2$ follows our mathematical argument, Theorem \ref{}. 

\subsubsection{Ratio of the height of $\rho_n(0)$ to $\rho_n(\bar x^{\max}_{n, M})$}
Next we study the ratio of the height of $\rho_n(0)$ to $\rho_n(\bar x^{\max}_{n, M})$.
As we see in Figure \ref{fig-dynamics_long_varM_1}, the height of the distributions among the center and the side looks almost identical for $M=2$, whereas it becomes significantly different for $M\geq 3$.
We have calculated the ratio $\rho_n(0)/\rho_n(\bar x^{\max}_{n, M})$ for various $M$.
In practical calculations, we have calculated the following average:
\begin{equation*}
\frac{1}{3000}\sum_{n=2001}^{5000}\frac{\rho_n(0)}{\rho_n(\bar x^{\max}_{n, M})}
\end{equation*}
as the ratio we are interested in.
Computation results are summarized in the row \lq\lq ratio" of Table \ref{Table-ch1}.
As indicated before, the ratio with $M=2$ is about $0.94$, which is approximately $1$, whereas the ratio drastically changes in $M\geq 3$ and we also see that the ratio stays at the range between $0.18$ and $0.2$ as $M$ increases.


\subsubsection{Asymptotic size of tail outside the limiting support}

Next we further study the nature of localized peaks.
A well-known result is that random walks followed by the normal distribution $N(0,1)$ has the probability distributions of the width $O(\sqrt{N})$, where $N$ is the number of iterations, while quantum walks typically have peak distribution of the width $O(N^{1/3})$ (cf. \cite{Sunada_Tate2012}).
To this end, we define the width $d_n$ of the tail distribution outside the peak of density as follows:
\begin{equation*}
d_n := a_n - \bar x^{\max}_{n, M},\quad \text{ where }\quad {\rm supp}\,\rho_n = [-a_n, a_n].
\end{equation*}
Assuming that $d_n$ follows the asymptotic behavior
\begin{equation*}
d_n \sim O(n^{\gamma_M})\quad \text{ as }\quad n\to \infty,
\end{equation*}
we calculate $\gamma_M$.
Computed results of $\gamma_M$ for various $M$ are shown in Table \ref{Table-ch1}.
We see that $\gamma_M$ converges to $1/3$ as $M$ increases, which indicates that the limiting behavior of the tail becomes close to well-known quantum walks according to e.g. \cite{Sunada_Tate2012}.

\subsubsection{Decay rate of $\rho_n(0)$ and $\rho_n(\bar x^{\max}_{n, M})$ as $n\to \infty$}
Finally we compute asymptotic decay rate of density $\rho_n$ inside the support.
More precisely, we assume the following asymptotic behavior
\begin{equation*}
\rho_n(x) \sim O(n^{d_M(x)})\quad \text{ as }\quad n\to \infty
\end{equation*}
and compute $d_M(x)$.
As representatives, we study the behavior of $\rho_n(0)$ and $\rho_n(\bar x^{\max}_{n, M})$.
Correspondingly we define
\begin{equation*}
d_M^{{\rm center}} := d_M(0),\quad d_M^{{\rm side}} := d_M(\bar x^{\max}_{n, M}).
\end{equation*}
Computation results are shown in Table \ref{Table-ch1}.
These results show that $d_M^{{\rm center}}$ becomes constant $1/2$, while $d_M^{{\rm side}}$ depends on $M$ in a nonlinear manner and converge to $-2/3$ as $M$ increases.


\begin{table}[ht]
\caption{Characteristics of off-diagonal peaks 1}
\centering
\begin{tabular}{c|cccccccc}
\hline
$M$ & $2$ & $3$ & $5$ & $10$ & $21$ & $51$ & $75$ & $101$ \\ [2mm]
\hline
$\bar x^{\max}_{M}$ & $0.5774$ & $0.6544$ & $0.6887$ & $0.7021$ & $0.6963$ & $0.6917$ & $0.6935$ & $0.6931$ \\ [2mm]
\hline
ratio & $0.9434$ & $0.2881$ & $0.1919$ & $0.2028$ & $0.1992$ & $0.1880$ & $0.1897$ & $0.1843$ \\ [2mm]
\hline
$\gamma_M$ & $0.4908$ & $0.4161$ & $0.3789$ & $0.3847$ & $0.7595$ & $0.3595$ & $0.3595$ & $0.3595$ \\[2mm]
\hline
$d_M^{{\rm center}}$ & $-0.4999$ & $-0.4998$ & $-0.4996$ & $-0.4992$ & $-0.4983$ & $-0.4959$ & $-0.4939$ & $-0.4919$ \\ [2mm]
\hline
$d_M^{{\rm side}}$ & $-0.4990$ & $-0.4830$ & $-0.3996$ & $-0.3368$ & $-0.4367$ & $-0.5811$ & $-0.6248$ & $-0.6563$ \\ [2mm]
\hline
\end{tabular}%
%}
\label{Table-ch1}\par
\end{table}

\begin{table}[ht]
\caption{Characteristics of off-diagonal peaks 2}
\centering
\begin{tabular}{c|ccccc}
\hline
$M$ & $126$ & $151$ & $175$ & $201$ & $226$ \\ [2mm]
\hline
$\bar x^{\max}_{M}$ & $0.7046$ & $0.7046$ & $0.7046$ & $0.7046$ & $0.7046$\\ [2mm]
\hline
ratio & $0.1514$ & $0.1379$ & $0.1277$ & $0.1188$ & $0.1117$ \\ [2mm]
\hline
$\gamma_M$ & $0.3507$ & $0.3507$ & $0.3507$ & $0.3507$ & $0.3507$ \\ [2mm]
\hline
$d_M^{{\rm center}}$ & $-0.4898$ & $-0.4877$ & $-0.4856$ & $-0.4834$ & $-0.4812$ \\ [2mm]
\hline
$d_M^{{\rm side}}$ & $-0.6564$ & $-0.6564$ & $-0.6564$ & $-0.6564$ & $-0.6564$ \\ [2mm]
\hline
\end{tabular}%
%}
\label{Table-ch2}\par
\end{table}

  

\subsection{Comparison with analytic results}
In $M=2$, we have obtained several analytic results for the asymptotic behavior of walkers.
\par
In the present section, we have chosen the vector $\phi^0 = (1/2,1/2,1/2,1/2,0,0,0,0)^T$ as the initial state.
We compute the decomposition of $\phi^0$ by eigenvectors $\phi_1, \phi_2, \phi_3$ for {\em unperturbed} matrix $\hat {\mathcal{W}}_{s,t}(0)$ computed in (\ref{ONB}) to study the net contribution of eigencomponents to dynamics of walkers.
We have
\begin{equation*}
(\phi^0, \phi_1) = 0,\quad (\phi^0, \phi_2) = \frac{1}{2\sqrt{3}},\quad (\phi^0, \phi_3) = \frac{1}{\sqrt{2}}
\end{equation*}
and
\begin{equation*}
\phi^0 = \frac{1}{2\sqrt{3}}\phi_2 +  \frac{1}{\sqrt{2}}\phi_3 + \left(-\frac{1}{12}, \frac{1}{2}, \frac{1}{3}, \frac{1}{12}, -\frac{1}{12}, -\frac{1}{6}, 0, \frac{1}{12}\right)^T
\end{equation*}

%\begin{align*}
%&\frac{1}{2} = (0*0 + \frac{1}{2\sqrt{3}} * \frac{1}{2\sqrt{3}} + \frac{1}{\sqrt{2}}*\frac{1}{\sqrt{2}} )\\
%&\frac{1}{2} = (0*0 + \frac{1}{2\sqrt{3}}*0 + \frac{1}{\sqrt{2}}*0)\\
%&\frac{1}{2} = (0*0 + \frac{1}{2\sqrt{3}}*\frac{1}{\sqrt{3}} + \frac{1}{\sqrt{2}}*0)\\
%&\frac{1}{2} = (0*0 + \frac{1}{2\sqrt{3}}* (-\frac{1}{2\sqrt{3}}) + \frac{1}{\sqrt{2}}*\frac{1}{\sqrt{2}} )\\
%&0 = (0*\frac{1}{\sqrt{2}}  + \frac{1}{2\sqrt{3}}* \frac{1}{2\sqrt{3}} + \frac{1}{\sqrt{2}}*0 )\\
%&0 = (0*\frac{1}{\sqrt{2}}  + \frac{1}{2\sqrt{3}}* \frac{1}{\sqrt{3}} + \frac{1}{\sqrt{2}}*0 )\\
%&0 = (0*\frac{1}{\sqrt{2}}  + \frac{1}{2\sqrt{3}}* 0 + \frac{1}{\sqrt{2}}*0 )\\
%&0 = (0*\frac{1}{\sqrt{2}}  + \frac{1}{2\sqrt{3}}* (-\frac{1}{2\sqrt{3}}) + \frac{1}{\sqrt{2}}*0 )\\
%\end{align*}




\subsection{Towards further discussions}
In this section we have studies dynamics of walkers via numerical simulations with various width $M$ of the underlying domain.
Our numerical results follow analytic results in the case $M=1,2$ discussed in the previous sections, and provides the possible nature of a crossover between open quantum random walks and quantum walks 

